Improving Object Detection via Local-global Contrastive Learning

Visual domain gaps often impact object detection performance. Image-to-image translation can mitigate this effect, where contrastive approaches enable learning of the image-to-image mapping under unsupervised regimes. However, existing methods often fail to handle content-rich scenes with multiple object instances, which manifests in unsatisfactory detection performance. Sensitivity to such instance-level content is typically only gained through object annotations, which can be expensive to obtain. Towards addressing this issue, we present a novel image-to-image translation method that specifically targets cross-domain object detection. We formulate our approach as a contrastive learning framework with an inductive prior that optimises the appearance of object instances through spatial attention masks, implicitly delineating the scene into foreground regions associated with the target object instances and background non-object regions. Instead of relying on object annotations to explicitly account for object instances during translation, our approach learns to represent objects by contrasting local-global information. This affords investigation of an under-explored challenge: obtaining performant detection, under domain shifts, without relying on object annotations nor detector model fine-tuning. We experiment with multiple cross-domain object detection settings across three challenging benchmarks and report state-of-the-art performance. Project page: https://local-global-detection.github.io

==> tables/KITTI_Sim10k_combined_v02.tex <==

%\begin{table}
\begin{adjustbox}{scale=0.5}
\begin{tabular}{l | c c | c c c c} 
\toprule
Method & D.A. & I2I    & car & person & mAP $\uparrow$  \\
\hline
DARL~\cite{Kim2019DiversifyAM} \textsc{\textit{{ }     (CVPR '19) }}  &{\hspace{0.2cm} \checkmark}  &{\hspace{0.05cm} \checkmark}  & 58.7 & 46.4& 52.5 \\
DAOD~\cite{DBLP:conf/bmvc/RodriguezM19} \textsc{\textit{{ }     (BMVC '19) }}  & {\hspace{0.2cm} \checkmark}  &{\hspace{0.05cm} \checkmark} & 59.1 & 47.3 &62.9  \\
DUNIT~\cite{bhattacharjee2020dunit} \textsc{\textit{{ }     (CVPR '20) }} & {\hspace{0.2cm} \checkmark} &{\hspace{0.05cm} \checkmark}  & 65.1 & \underline{60.7} &62.9 \\
MGUIT \cite{9577366} \textsc{\textit{{ }     (CVPR '21) }}  & &{\hspace{0.05cm} \checkmark}  & 68.2 & 58.3 & 63.2\\
InstaFormer~\cite{kim2022instaformer} \textsc{\textit{{ }     (CVPR '22) }}  & &{\hspace{0.05cm} \checkmark}  & \underline{69.5} & \textbf{61.8} & \textbf{65.6}\\
DA-DETR~\cite{Zhang2021DADETRDA} \textsc{\textit{{ }     (CVPR '22) }}  & &{\hspace{0.05cm} \checkmark}  &  48.9 & - & - \\
\hline
Source &&& 63.4 & 55.0 & 59.2 \\
Target Oracle  &&& 77.4 & 66.3 & 71.8  \\
Ours - supervised   &   &{\hspace{0.05cm} \checkmark} & \textbf{71.0} & 59.5 & \underline{65.2} \\ 
Ours - local-global $^\dag$   & &{\hspace{0.05cm} \checkmark} & 67.5 & \underline{60.7} & 64.1 \\ 
\bottomrule     
\end{tabular}
\end{adjustbox}

%\hspace{0.5cm}


\begin{adjustbox}{scale=0.5}
\begin{tabular}{l | c c c | c} 
\toprule
Method & D.A. & I2I  & Backbone & $AP_{car} \uparrow$  \\
\hline
HTCN~\cite{chen2020harmonizing} \textsc{\textit{{ }     (CVPR '20) }} & {\hspace{0.7cm} \checkmark}& {  \checkmark}&Vgg-16& 42.5\\
UMT~\cite{deng_li_chen_duan_2021}   \textsc{\textit{{ }     (CVPR '21) }} & {\hspace{0.7cm} \checkmark} & {  \checkmark}   &Vgg-16&  43.1\\
FGRR~\cite{DBLP:journals/pami/ChenLZHHDY23} \textsc{\textit{{ }     (PAMI '23) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 44.5\\ 
DSS~\cite{wang2021domain} \textsc{\textit{{ }     (CVPR '21) }}  &  {\hspace{0.7cm} \checkmark}  & &Res-50 & 44.5 \\
SWDA~\cite{saito_ushiku_harada_saenko_2019} \textsc{\textit{{ }     (CVPR '19) }}  & {\hspace{0.7cm} \checkmark}  & &Res-50  & 44.6\\
SCDA~\cite{zhu_pang_yang_shi_lin_2019} \textsc{\textit{{ }     (CVPR '19) }}   & {\hspace{0.7cm} \checkmark}  & &Res-50&   45.1 \\
AFAN~\cite{wang_liao_shao_2021} \textsc{\textit{{ }     (TIP '21) }} & {\hspace{0.7cm} \checkmark}  &   {  \checkmark}& Res-50 & 45.5\\
GPA~\cite{xu2020cross} $(CVPR '20)$  &  {\hspace{0.7cm} \checkmark}   &    & Res-50 & 47.6 \\
SDA~\cite{rezaeianaran2021seeking} \textsc{\textit{{ }     (CVPR '21) }} &{\hspace{0.7cm} \checkmark}&    & Vgg-16& 49.3  \\
MGA~\cite{DBLP:journals/pami/ChenLZHHDY23} \textsc{\textit{{ }     (CVPR '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 49.8\\
KTNet~\cite{9710025} \textsc{\textit{{ }     (ICCV '21) }}&  {\hspace{0.7cm} \checkmark} &&Vgg-16& 50.7 \\
SSAL~\cite{Munir2021SynergizingBS} \textsc{\textit{{ }     (NeurIPS '21) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 51.8\\
SCAN~\cite{DBLP:conf/aaai/LiLYY22} \textsc{\textit{{ }     (AAAI '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 52.6\\
SIGMA~\cite{li2022sigma} \textsc{\textit{{ }     (CVPR '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 53.4\\
DA-DETR~\cite{Zhang2021DADETRDA} \textsc{\textit{{ }     (CVPR '23) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& \textbf{54.7}\\
\hline
\emph{Source} & && Res-50 & 41.7 \\
Ours - supervised ($\Lb_{G_{A_{sup}}}$) & &{  \checkmark}& Res-50 &  \underline{53.6} \\ 
Ours -  local-global $^{\dag}$   & &{  \checkmark}& Res-50 & 52.1 \\ 
\bottomrule
\end{tabular} 
\end{adjustbox}

\caption{Adaptation results for KITTI $\rightarrow$ Cityscapes (left) and Sim10K $\rightarrow$ Cityscapes (right). }
\label{tab:results:sim_kitt_combined}

%\end{table}







==> tables/KITTI_to_cityscapes_v01.tex <==
\begin{table}[ht]
\footnotesize
\setlength\tabcolsep{4pt}
%\setlength{\tabcolsep}{2pt}
\centering
\begin{adjustbox}{scale=0.77}
%\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} c | c | c c c c c c c c | c c}
\begin{tabular}{l | c c |c c c c} 
%\multicolumn{12}{c}{\Large{ Domain-Adaptive Object Detection }} \\
\toprule
Method & Detector adaptation & I2I translation   & car & person & mAP $\uparrow$  \\
\hline
%DT~\cite{inoue2018cross} \textsc{\textit{{\hspace{0.2cm}}     (CVPR '18) }} &{\hspace{0.2cm} \checkmark}  &{\hspace{0.05cm} \checkmark}  & 40.7 & 28.5 &34.6\\
%DAF \cite{huang2018munit} \textsc{\textit{{\hspace{0.2cm}}     (CVPR '17) }}  & {\hspace{0.2cm} \checkmark}  &{\hspace{0.05cm} \checkmark} &40.2 & 39.2 & 39.7\\
DARL~\cite{Kim2019DiversifyAM} \textsc{\textit{{ }     (CVPR '19) }}  &{\hspace{0.2cm} \checkmark}  &{\hspace{0.05cm} \checkmark}  & 58.7 & 46.4& 52.5 \\
DAOD~\cite{DBLP:conf/bmvc/RodriguezM19} \textsc{\textit{{ }     (BMVC '19) }}  & {\hspace{0.2cm} \checkmark}  &{\hspace{0.05cm} \checkmark} & 59.1 & 47.3 &62.9  \\
DUNIT~\cite{bhattacharjee2020dunit} \textsc{\textit{{ }     (CVPR '20) }} & {\hspace{0.2cm} \checkmark} &{\hspace{0.05cm} \checkmark}  & 65.1 & \underline{60.7} &62.9 \\
 MGUIT \cite{9577366} \textsc{\textit{{ }     (CVPR '21) }}  & &{\hspace{0.05cm} \checkmark}  & 68.2 & 58.3 & 63.2\\
 InstaFormer~\cite{kim2022instaformer} \textsc{\textit{{ }     (CVPR '22) }}  & &{\hspace{0.05cm} \checkmark}  & \underline{69.5} & \textbf{61.8} & \textbf{65.6}\\
 \hline
 Source &&& 63.4 & 55.0 & 59.2 \\
 Target Oracle  &&& 77.4 & 66.3 & 71.8  \\
Ours - supervised   &   &{\hspace{0.05cm} \checkmark} & \textbf{71.0} & 59.5 & \underline{65.2} \\ 
 Ours - local-global $^\dag$   & &{\hspace{0.05cm} \checkmark} & 67.5 & \underline{60.7} & 64.1 \\ 

 DA-DETR~\cite{Zhang2021DADETRDA} \textsc{\textit{{ }     (CVPR '22) }}  & &{\hspace{0.05cm} \checkmark}  &  48.9 & - & - \\
 \hline
 
 Source &&& 63.4 & 55.0 & 59.2 \\
 Target Oracle  &&& 77.4 & 66.3 & 71.8  \\
Ours - supervised ($\Lb_{G_{A_{sup}}}$)  &   &{\hspace{0.05cm} \checkmark} & \textbf{71.0} & 59.5 & \underline{65.2} \\ 
 Ours - local-global $^\dag$   & &{\hspace{0.05cm} \checkmark} & 67.5 & \underline{60.7} & 64.1 \\ 


%% Our results

%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
%  Multilevel knowledge transfer for crossdomain object detection
% 50.2 whats the venue ?
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% Cross-Domain Adaptive Teacher for Object Detection -*** uses ResNet 101 backbone for detector
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% H2FA R-CNN: Holistic and Hierarchical Feature Alignment for Cross-domain Weakly Supervised Object Detection -*** Does not report foggy citycsapes results in table (only in barplots)
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% Cross Domain Object Detection by Target-Perceived Dual Branch Distillation - *** uses FPN in detector backbone that gives around +5-6 % mAP & performs inference on larger resolution so it is largerly unfair 
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% https://arxiv.org/pdf/2212.01322v1.pdf - MIC: Masked Image Consistency for Context-Enhanced Domain Adaptation  - has it been published somewhere ? mAP 47.6 
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------



\\

%bus bcycle car cycle person rider train truck mAP
%(\textit{Ours}) &  & - & - & - & - & - & - & - & - & \textbf{46.9} & - \\



\end{tabular}
\end{adjustbox}
\caption{Adaptation results for KITTI $\rightarrow$ Cityscapes. }

\label{tab:results:kitti} 
\end{table}

==> tables/KITTI_to_cityscapes_v02.tex <==
\begin{adjustbox}{scale=0.5}
\begin{tabular}{l | c c | c c c c} 
\toprule
Method & D.A. & I2I    & car & person & mAP $\uparrow$  \\
\hline
DARL~\cite{Kim2019DiversifyAM} \textsc{\textit{{ }     (CVPR '19) }}  &{\hspace{0.2cm} \checkmark}  &{\hspace{0.05cm} \checkmark}  & 58.7 & 46.4& 52.5 \\
DAOD~\cite{DBLP:conf/bmvc/RodriguezM19} \textsc{\textit{{ }     (BMVC '19) }}  & {\hspace{0.2cm} \checkmark}  &{\hspace{0.05cm} \checkmark} & 59.1 & 47.3 &62.9  \\
DUNIT~\cite{bhattacharjee2020dunit} \textsc{\textit{{ }     (CVPR '20) }} & {\hspace{0.2cm} \checkmark} &{\hspace{0.05cm} \checkmark}  & 65.1 & \underline{60.7} &62.9 \\
MGUIT \cite{9577366} \textsc{\textit{{ }     (CVPR '21) }}  & &{\hspace{0.05cm} \checkmark}  & 68.2 & 58.3 & 63.2\\
InstaFormer~\cite{kim2022instaformer} \textsc{\textit{{ }     (CVPR '22) }}  & &{\hspace{0.05cm} \checkmark}  & \underline{69.5} & \textbf{61.8} & \textbf{65.6}\\
DA-DETR~\cite{Zhang2021DADETRDA} \textsc{\textit{{ }     (CVPR '22) }}  & &{\hspace{0.05cm} \checkmark}  &  48.9 & - & - \\
\hline
Source &&& 63.4 & 55.0 & 59.2 \\
Target Oracle  &&& 77.4 & 66.3 & 71.8  \\
Ours - supervised   &   &{\hspace{0.05cm} \checkmark} & \textbf{71.0} & 59.5 & \underline{65.2} \\ 
Ours - local-global $^\dag$   & &{\hspace{0.05cm} \checkmark} & 67.5 & \underline{60.7} & 64.1 \\ 
\bottomrule     
\end{tabular}
\end{adjustbox}
\caption{KITTI $\rightarrow$ Cityscapes. }
\label{tab:results:kitti} 

==> tables/foggy_cityscapes_to_cityscapes_v01.tex <==
\begin{table}[ht]

%\footnotesize
\setlength\tabcolsep{5pt}
%\centering
%\begin{adjustbox}{scale=0.70}
\begin{tabular*}{}%{@{\extracolsep{\fill}} l  | l l l | c c c c c c c c c c c c c | c c}
%\begin{tabular}{c | c | c c c c c c c c | c c} 
%\multicolumn{12}{c}{\Large{ Domain-Adaptive Object Detection }} \\
%\hline
\toprule
Method  & D.A. & I2I  &  Backbone &  person & rider & car & truck & bus & train & motor & bike & mAP $\uparrow$   \\
%\hline
% CFFA~\cite{zheng2020cross} $(CVPR'20)$    & \multirow{9}{*}{Vgg-16-16} & 34.0 & 46.9 & 52.1 & 30.8 & 43.2 & 29.9 & 34.7 & 37.4 & 38.6  \\
% EPM~\cite{hsu2020every} $(ECCV'20)$       &                         & 41.9 & 38.7 & 56.7 & 22.6 & 41.5 & 26.8 & 24.6 & 35.5 & 36.0 \\
% RPNPA~\cite{zhang2021rpn} $(CVPR'21)$     &                         & 33.6 & 43.8 & 49.6 & 32.9 & 45.5 & 46.0 & 35.7 & 36.8 & 40.5  \\
% UMT~\cite{deng2021unbiased} $(CVPR'21)$   &                         & 33.0 & 46.7 & 48.6 & 34.1 & 56.5 & 46.8 & 30.4 & 37.4 & 41.7 \\
% MeGA~\cite{vs2021mega} $(CVPR'21)$        &                         & 37.7 & 49.0 & 52.4 & 25.4 & 49.2 & 46.9 & 34.5 & 39.0 & 41.8  \\
% ICCR-VDD~\cite{wu2021vector} $(ICCV'21)$  &                         & 33.4 & 44.0 & 51.7 & 33.9 & 52.0 & 34.7 & 34.2 & 36.8 & 40.0  \\
% KTNet~\cite{tian2021knowledge} $(ICCV'21)$&                         & 46.4 & 43.2 & 60.6 & 25.8 & 41.2 & 40.4 & 30.7 & 38.8 & 40.9  \\
% SSAL~\cite{munir2021ssal} $(NeurIPS'21)$  &                         & 45.1 & 47.4 & 59.4 & 24.5 & 50.0 & 25.7 & 26.0 & 38.7 & 39.6 \\
% SIGMA~\cite{li2022sigma} $(CVPR'22)$      &                         & 46.9 & 48.4 & 63.7 & 27.1 & 50.7 & 35.9 & 34.7 & 41.4 & 43.5  \\
CDTD~\cite{shen2021cdtd}   \textsc{\textit{{ }     (IJCV '21) }}       &  {\hspace{0.1cm} \checkmark}    &    {\hspace{0.1cm} \checkmark}           &Vgg-16& 31.6 & 44.0 & 44.8 & 30.4 & 41.8 & 40.7 & 33.6 & 36.2 & 37.9 & \\
%GPA~\cite{xu2020cross}          \textsc{\textit{{\hspace{0.2cm}}     (CVPR '20) }}  & {\hspace{0.1cm} \checkmark} &     &Res-50& 32.9 & 46.7 & 54.1 & 24.7 & 45.7 & 41.1 & 32.4 & 38.7 & 39.5  \\
%EPM~\cite{hsu2020every}       \textsc{\textit{{\hspace{0.2cm}}     (ECCV '20) }} &  {\hspace{0.1cm} \checkmark}      &                            &Res-50& 39.9 & 38.1 & 57.3 & 28.7 & 50.7 & 37.2 & 30.2 & 34.2 & 39.5  \\
AFAN~\cite{wang_liao_shao_2021}         \textsc{\textit{{ }     (TIP '21) }} &  {\hspace{0.1cm} \checkmark}        &{\hspace{0.1cm} \checkmark} &Res-50& 42.5 & 44.6& 57.0& 26.4& 48.0& 28.3& 33.2& 37.1& 39.6 \\
HTCN~\cite{chen2020harmonizing}  \textsc{\textit{{ }     (CVPR '20) }} & {\hspace{0.1cm} \checkmark}         &  {\hspace{0.1cm} \checkmark}     &             Vgg-16&    33.2& 47.5& 47.9& 31.6& 47.4& 40.9& 32.3& 37.1  & 39.8   \\
%DIDN~\cite{lin2021domain}     \textsc{\textit{{\hspace{0.2cm}}     (ICCV '21) }} & {\hspace{0.1cm} \checkmark}         &                           &Res-50& 38.3 & 44.4 & 51.8 & 28.7 & 53.3 & 34.7 & 32.4 & 4.4 & 40.5  \\
FGRR~\cite{DBLP:journals/pami/ChenLZHHDY23}     \textsc{\textit{{ }     (TPAMI'23) }}          & {\hspace{0.1cm} \checkmark}    &                            &Vgg-16& 34.4 &47.6 & 51.3 &30.0& 46.8 & 42.3 & 35.1 & 38.9 & 40.8 \\
DSS~\cite{wang2021domain}  \textsc{\textit{{ }     (CVPR '21) }} &   {\hspace{0.1cm} \checkmark}         &                               &Res-50& 42.9 & 51.2 & 53.6 & 33.6 & 49.2 & 18.9 & 36.2 & 41.8 & 40.9 \\
UMT~\cite{deng_li_chen_duan_2021}   \textsc{\textit{{ }     (CVPR '21) }}  & {\hspace{0.1cm} \checkmark}     &       {\hspace{0.1cm} \checkmark}           &Vgg-16& 33.0 & 46.7 & 48.6 & 34.1 & 56.5 & 46.8& 30.4 & 37.3 & 41.7 & \\
DAF+NLTE~\cite{liu_li_yang_li_yuan_2022}  \textsc{\textit{{ }     (CVPR '22) }} & {\hspace{0.1cm} \checkmark}            &                            &Res-50& 37.0 & 46.9 & 54.8 & 32.1 & 49.9 & 43.5 & 29.9 & 39.6 & 41.8  \\
TIA~\cite{zhao_wang_2022}     \textsc{\textit{{ }     (CVPR '22) }}    & {\hspace{0.1cm} \checkmark}    &          {\hspace{0.1cm} \checkmark}                    &Res-50& 34.8 & 46.3& 49.7 & 31.1 & 52.1  & 48.6 & 37.7 & 38.1 & 42.3  \\
SCAN~\cite{DBLP:conf/aaai/LiLYY22}     \textsc{\textit{{ }     (AAAI '22) }}          & {\hspace{0.1cm} \checkmark}    &                            &Vgg-16& 41.7 & 43.9 & 57.3 & 28.7& 48.6& 48.7& 31.0 &37.3 &42.1\\
SIGMA~\cite{li2022sigma}     \textsc{\textit{{ }     (CVPR '22) }}          & {\hspace{0.1cm} \checkmark}    &                            &Res-50& 46.9 &48.4& {63.7} & 27.1& 50.7& 35.9& 34.7& 41.4& 43.5 \\
SDA~\cite{rezaeianaran2021seeking}  \textsc{\textit{{ }     (CVPR '21) }}   & {\hspace{0.1cm} \checkmark}    &                           &Res-50& 38.8 & 45.9 & 57.2 & 29.9 & 50.2 & 51.9 & 31.9 & 40.9 & 43.3 & \\

MGA~\cite{Zhou2022MultiGranularityAD}     \textsc{\textit{{ }     (CVPR '22) }}          & {\hspace{0.1cm} \checkmark}    &                            &Vgg-16& 43.9 & 49.6 & 60.6 & 29.6 & 50.7 & 39.0 & 38.3 & 42.8  & 44.3 \\

DA-DETR~\cite{Zhang2021DADETRDA}     \textsc{\textit{{ }     (CVPR '23) }}          & {\hspace{0.1cm} \checkmark}    &                            &Res-50& 49.9 & 50.0 & 63.1 & 24.0 & 45.8 & 37.5 & 31.6 & 46.3 & 43.5 \\

%$O^2$Net~\cite{Zhang2021DADETRDA}     \textsc{\textit{{ }     (AMC '22) }}          & {\hspace{0.1cm} \checkmark}    &                            &Vgg-16& 48.7 & 51.5 & 63.6 & 31.1 & 47.6 & 47.8 & 38.0 & 45.9  & 46.8 \\

memCLR~\cite{Vibashan2022TowardsOD}     \textsc{\textit{{ }     (WACV'23) }}          & {\hspace{0.1cm} \checkmark}    &                            &Vgg-16& 37.7 & 42.8& 52.4& 24.5& 40.6&31.7 & 29.4 & 42.2  & 37.7 \\


MIC~\cite{Hoyer2022MICMI}     \textsc{\textit{{ }     (CVPR 23) }}          & {\hspace{0.1cm} \checkmark}    &                            &Vgg-16& 

52.4 &47.5 &67.0 &40.6 &50.9 &55.3 &33.7 &33.9 & \underline{47.6} \\

CDAT~\cite{Cao2023ContrastiveMT}     \textsc{\textit{{ }     (CVPR 23) }}          & {\hspace{0.1cm} \checkmark}    &                            &Vgg-16& 
42.3 &51.7 &64.0 &26.0 &42.7 &37.1 &42.5 &44.0& 43.8 \\


NSA-UDA~\cite{NSAUDA}     \textsc{\textit{{ }     (ICCV 23) }}          & {\hspace{0.1cm} \checkmark}    &                            &Vgg-16& - & - & - & - & - & - & - & - & \textbf{52.7}\\
% SIGMA++ ~\cite{li_liu_yuan_2023}  \textsc{\textit{{\hspace{0.2cm}}     (TPAMI '23) }}  & {\hspace{0.1cm} \checkmark}    && Vgg-16&        46.4 &45.1& 61.0& 32.1 &52.2& 44.6& 34.8& 39.9& 44.5   
%  \\

\midrule
\midrule
%\hline 
%\hline
CUT$^{*\dag}$~\cite{park2020contrastive} \textsc{\textit{{ }     (ECCV '20) }} & &  {\hspace{0.1cm} \checkmark}     &      Res-50& 39.6 & 45.3 & 59.4 & 27.9 &47.4 & 45.4 &35.3 &39.2& 42.4    &             \\
FeSeSim$^{*\dag}$~\cite{zheng_cham_cai_2021}  \textsc{\textit{{ }     (CVPR '21) }}       &&  {\hspace{0.1cm} \checkmark}  &   Res-50& 40.9 &47.2 &58.4 &28.4 &48.6 &49.8 &34.3 &42.7 &43.8            \\
Qs-Att.$^{*\dag}$~\cite{hu_zhou_huang_shi_sun_li_2022}  \textsc{\textit{{ }     (CVPR '22) }}       &&      {\hspace{0.1cm} \checkmark}  & Res-50&                     42.2 & 49.0 &60.3 & 23.5 & 50.5  & 52.0  &36.6  & 41.4 & 44.4   \\

%OrderedDict([('bbox', {'AP': 23.48515584548298, 'AP50': 44.25097493476278, 'AP75': 22.031802185626397, 'APs': 2.7366894356435845, 'APm': 21.317796045667727, 'APl': 46.3882587816449, 'AP-person': 42.20388359273407, 'AP-car': 58.84025561123967, 'AP-train': 50.213323440072344, 'AP-rider': 48.2425495203324, 'AP-truck': 27.972535284282724, 'AP-motorcycle': 34.92923212426565, 'AP-bicycle': 43.76202833781789, 'AP-bus': 47.84399156735752})])


NEGCUT$^{*\dag}$~\cite{negcut}  \textsc{\textit{{ }     (CVPR '21) }}       &&      {\hspace{0.1cm} \checkmark}  & Res-50&                     42.2 & 48.2 &58.8 & 27.9 & 47.8  & 50.2  &34.9  & 43.7 & 44.2   \\


%OrderedDict([('bbox', {'AP': 23.59650731091053, 'AP50': 44.970816532017786, 'AP75': 22.07462735715705, 'APs': 2.74477759092647, 'APm': 22.35083714768246, 'APl': 46.72038666836867, 'AP-person': 42.86677706110227, 'AP-car': 59.73095018906221, 'AP-train': 48.983996971783775, 'AP-rider': 46.96846499977767, 'AP-truck': 32.35927600207285, 'AP-motorcycle': 36.8888661320815, 'AP-bicycle': 43.48313729771207, 'AP-bus': 48.48506360254989})])


Hneg\_SCR$^{*\dag}$~\cite{hneg}  \textsc{\textit{{ }     (CVPR '22) }}       &&      {\hspace{0.1cm} \checkmark}  & Res-50&                     42.8 & 46.9 & 59.7 & 32.3 & 48.4  & 48.9  & 36.8  & 43.4 & 44.9   \\



%OrderedDict([('bbox', {'AP': 24.0418267196259, 'AP50': 45.19052139121265, 'AP75': 22.722171929241203, 'APs': 2.6071680101163035, 'APm': 22.564777470766185, 'APl': 47.455461167690046, 'AP-person': 42.351290804115074, 'AP-car': 59.4936671809552, 'AP-train': 49.1501785646545, 'AP-rider': 47.944020242682285, 'AP-truck': 34.407310888762375, 'AP-motorcycle': 36.487631129454975, 'AP-bicycle': 42.31469436586077, 'AP-bus': 49.375377953216045})])



Santa$^{*\dag}$~\cite{santa}  \textsc{\textit{{ }     (CVPR '23) }}       &&      {\hspace{0.1cm} \checkmark}  & Res-50&                     42.3 & 47.9 & 59.4 & 34.4 & 49.3  & 49.1  &36.4  & 42.3 & \underline{45.1}   \\


\midrule
\emph{Source}            &&&          Res-50                & 35.5 & 38.7 & 41.5 & 18.4 & 32.8 & 12.5 & 22.3 & 33.6 & 29.4 &  \\
\emph{Target Oracle}          & &&          Res-50                &47.5& 51.7 & 66.9 & 39.4 & 56.8  & 49.0 & 43.2 & 47.3 & 50.2   \\
Ours - supervised ($\Lb_{G_{A_{sup}}}$)           & & {\hspace{0.1cm} \checkmark} &          Res-50                & 44.4  &49.5& 61.4 & 32.6 & 50.8 & 52.2 & 38.3 & 44.0 & {46.7}&  \\
Ours - local-global $^{\dag}$             &  & {\hspace{0.1cm} \checkmark} &        Res-50             & 43.2 & 50.1 & 61.7 & 33.3 & 48.6  & 47.8 & 35.2 & 42.6 & \textbf{45.3}&  \\


\bottomrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CUT final %%%%%%%%%%%%%%%V%%%%%

% OrderedDict([('bbox', {'AP': 22.36457370101299, 'AP50': 42.48892947597932, 'AP75': 20.794039775739726, 'APs': 2.228625241053333, 'APm': 21.4065676679617, 'APl': 45.00610353788152, 'AP-person': 39.64674782972589, 'AP-car': 59.41188579571024, 'AP-train': 45.49074472664658, 'AP-rider': 45.32119793301533, 'AP-truck': 27.989533021171308, 'AP-motorcycle': 35.35548548284645, 'AP-bicycle': 39.219567493470194, 'AP-bus': 47.476273525248544})])

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FeSeSim %%%%%%%%%%%%%%%V%%%%%

% OrderedDict([('bbox', {'AP': 22.97256578108796, 'AP50': 43.84813963450197, 'AP75': 21.045324283523705, 'APs': 2.178378322735707, 'APm': 21.47228591808014, 'APl': 46.926413509658914, 'AP-person': 40.93232241313784, 'AP-car': 58.436626585032606, 'AP-train': 49.87481506771367, 'AP-rider': 47.28383559549671, 'AP-truck': 28.457864916772323, 'AP-motorcycle': 34.449330498947766, 'AP-bicycle': 42.725153891649974, 'AP-bus': 48.62516810726484})])

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% QS-ATN %%%%%%%%%%%%%%%V%%%%%

%OrderedDict([('bbox', {'AP': 24.1 
 % Ours - scheme II   & 51.3 \\ 92081518053016, 'AP50': 44.49695383227811, 'AP75': 21.831627609138447, 'APs': 2.716230447697815, 'APm': 22.225077558018523, 'APl': 46.93632198628181, 'AP-person': 42.29073396559132, 'AP-car': 60.37830183735069, 'AP-train': 52.06118618506369, 'AP-rider': 49.013964375226045, 'AP-truck': 23.562624311480683, 'AP-motorcycle': 36.65480191709296, 'AP-bicycle': 41.43231705870667, 'AP-bus': 50.58170100771279})])

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  OURS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% OrderedDict([('bbox', {'AP': 16.513763238504293, 'AP50': 29.472439612412533, 'AP75': 15.983415858451098, 'APs': 0.7062978376258716, 'APm': 15.430939629533905, 'APl': 39.61299781230368, 'AP-person': 35.543124312665924, 'AP-car': 41.584567781555606, 'AP-train': 12.547978057568066, 'AP-rider': 38.77983463199229, 'AP-truck': 18.4816324422593, 'AP-motorcycle': 22.34841664656414, 'AP-bicycle': 33.690758455301776, 'AP-bus': 32.803204571393174})])

%OrderedDict([('bbox', {'AP': 26.51202224831976, 'AP50': 50.270146170453366, 'AP75': 24.83248858462606, 'APs': 3.6972689879187386, 'APm': 26.869467333264968, 'APl': 49.26411633553484, 'AP-person': 47.50448980470352, 'AP-car': 66.96933671613264, 'AP-train': 49.0909320669123, 'AP-rider': 51.79263132022327, 'AP-truck': 39.401034821708556, 'AP-motorcycle': 43.28440341648893, 'AP-bicycle': 47.316496813706706, 'AP-bus': 56.801844403751})])

%OrderedDict([('bbox', {'AP': 24.132713257761793, 'AP50': 45.35974552394747, 'AP75': 23.25165492233771, 'APs': 2.6453827460346258, 'APm': 23.380161857018418, 'APl': 47.15062219209136, 'AP-person': 43.26549984328365, 'AP-car': 61.75554940961949, 'AP-train': 47.879585680345095, 'AP-rider': 50.145423742067244, 'AP-truck': 33.29353831969976, 'AP-motorcycle': 35.23515823787455, 'AP-bicycle': 42.65072513622375, 'AP-bus': 48.65248382246621})])

%OrderedDict([('bbox', {'AP': 24.575586359212856, 'AP50': 46.709232246424804, 'AP75': 22.964798436094956, 'APs': 2.740371096869336, 'APm': 23.45720275912138, 'APl': 47.10225438662094, 'AP-person': 44.44898307438556, 'AP-car': 61.44584956658543, 'AP-train': 52.28409718799934, 'AP-rider': 49.509519369625565, 'AP-truck': 32.67285643256479, 'AP-motorcycle': 38.36503091677964, 'AP-bicycle': 44.08183362895964, 'AP-bus': 50.86568779449851})])



%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
%  Towards Robust Adaptive Object Detection under Noisy Annotations
%  
%                  prsn rider car truck bus train mtor bike 
% DAF+NLTE (Ours)† 43.1 50.7 58.7 33.6 56.7 42.7 33.7 43.3 45.4
% DAF+NLTE (Ours) 37.0 46.9 54.8 32.1 49.9 43.5 29.9 39.6 41.8
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% Cross-Domain Adaptive Teacher for Object Detection -*** uses ResNet 101 backbone for detector
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% H2FA R-CNN: Holistic and Hierarchical Feature Alignment for Cross-domain Weakly Supervised Object Detection -*** Does not report foggy citycsapes results in table (only in barplots)
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% Cross Domain Object Detection by Target-Perceived Dual Branch Distillation - *** uses FPN in detector backbone that gives around +5-6 % mAP & performs inference on larger resolution so it is largerly unfair 
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% https://arxiv.org/pdf/2212.01322v1.pdf - MIC: Masked Image Consistency for Context-Enhanced Domain Adaptation  - has it been published somewhere ? mAP 47.6 
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------

%bus bcycle car cycle person rider train truck mAP
%(\textit{Ours}) &  & - & - & - & - & - & - & - & - & \textbf{46.9} & - \\

\end{tabular*}
%\end{adjustbox}
\caption{The Foggy Cityscapes $\rightarrow$ Cityscapes adaptation scenario. We report object detection (mAP) per class. %results both per-class and via mean average precision (mAP). We indicate where 
Previous works utilises detector adaptation (D.A), image-to-image translation (I2I) components. Locally reproduced methods using publicly available codes are indicated by \textbf{*}. We separate methods that \textbf{do} (upper) and \textbf{do not} (lower) have access to object annotations at training time, with the latter methods denoted $\mathbf{\dag}$. Results are denoted \textbf{best} and \underline{second best}.}% for upper and lower table sections.} 
\label{tab:results:foggy} 
\end{table}

% \caption{The Foggy Cityscapes $\rightarrow$ Cityscapes adaptation scenario. We report the usage of an image-to-image translation module and detector backbone network type. *indicates locally produced results, \dag indicates that the method does not assume access to object annotations during training  }

==> tables/sim10k_to_cityscapes_v01.tex <==
\begin{table}[ht]
\footnotesize
\setlength\tabcolsep{4pt}
%\setlength{\tabcolsep}{2pt}
\centering
\begin{adjustbox}{scale=0.75}
%\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} c | c | c c c c c c c c | c c}
\begin{tabular}{l | c c c | c} 
%\multicolumn{12}{c}{\Large{ Domain-Adaptive Object Detection }} \\
\toprule
Method & Detector adaptation & I2I translation & Backbone & $AP_{car} \uparrow$  \\
\hline
 %D\&Match \cite{kim_jeong_kim_choi_kim_2019} \textsc{\textit{{ }     (CVPR '19) }} & && &43.9 \\

  HTCN~\cite{chen2020harmonizing} \textsc{\textit{{ }     (CVPR '20) }} & {\hspace{0.7cm} \checkmark}& {  \checkmark}&Vgg-16& 42.5
 \\
  UMT~\cite{deng_li_chen_duan_2021}   \textsc{\textit{{ }     (CVPR '21) }} & {\hspace{0.7cm} \checkmark} & {  \checkmark}   &Vgg-16&  43.1\\
   FGRR~\cite{DBLP:journals/pami/ChenLZHHDY23} \textsc{\textit{{ }     (PAMI '23) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 44.5
 \\ 
 DSS~\cite{wang2021domain} \textsc{\textit{{ }     (CVPR '21) }}  &  {\hspace{0.7cm} \checkmark}  & &Res-50 & 44.5 \\
SWDA~\cite{saito_ushiku_harada_saenko_2019} \textsc{\textit{{ }     (CVPR '19) }}  & {\hspace{0.7cm} \checkmark}  & &Res-50  & 44.6\\
SCDA~\cite{zhu_pang_yang_shi_lin_2019} \textsc{\textit{{ }     (CVPR '19) }}   & {\hspace{0.7cm} \checkmark}  & &Res-50&   45.1 \\
AFAN~\cite{wang_liao_shao_2021} \textsc{\textit{{ }     (TIP '21) }} & {\hspace{0.7cm} \checkmark}  &   {  \checkmark}& Res-50 & 45.5\\
 GPA~\cite{xu2020cross} $(CVPR '20)$  &  {\hspace{0.7cm} \checkmark}   &    & Res-50 & 47.6 \\
 SDA~\cite{rezaeianaran2021seeking} \textsc{\textit{{ }     (CVPR '21) }} &{\hspace{0.7cm} \checkmark}&    & Vgg-16& 49.3  \\
  MGA~\cite{DBLP:journals/pami/ChenLZHHDY23} \textsc{\textit{{ }     (CVPR '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 49.8
 \\
 KTNet~\cite{9710025} \textsc{\textit{{ }     (ICCV '21) }}&  {\hspace{0.7cm} \checkmark} &&Vgg-16& 50.7 \\
 SSAL~\cite{Munir2021SynergizingBS} \textsc{\textit{{ }     (NeurIPS '21) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 51.8
 \\
   SCAN~\cite{DBLP:conf/aaai/LiLYY22} \textsc{\textit{{ }     (AAAI '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 52.6
 \\
  SIGMA~\cite{li2022sigma} \textsc{\textit{{ }     (CVPR '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 53.4
 \\

DA-DETR~\cite{Zhang2021DADETRDA} \textsc{\textit{{ }     (CVPR '23) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& \textbf{54.7}
 \\
% SIGMA~\cite{li2022sigma}     \textsc{\textit{{ }     (CVPR '22) }}          & {\hspace{0.7cm} \checkmark}    &                            &Res-50& 46.9 &48.4& 63.7& 27.1& 50.7& 35.9& 34.7& 41.4& 43.5 \\
 
% HTCN \cite{chen_zheng_ding_huang_dou_2020}  \textsc{\textit{{ }     (CVPR '20) }} & {\hspace{0.7cm} \checkmark}         & 
 
% MGA~\cite{Zhou2022MultiGranularityAD}     \textsc{\textit{{ }     (CVPR '22) }}          & {\hspace{0.7cm} \checkmark}    &                            &Res-50& 43.9 & 49.6 & 60.6 & 29.6 & 50.7 & 39.0 &38.3 & 42.8  &44.3 \\

% MKT \cite{Csaba2021MultilevelKT} \textsc{\textit{{ }     (ICCVW '22) }}  & && Res-50& 50.2 \\

\hline
\emph{Source} & && Res-50 & 41.7 \\
Ours - supervised & &{  \checkmark}& Res-50 &  \underline{53.6} \\ 
Ours -  local-global $^{\dag}$   & &{  \checkmark}& Res-50 & 52.1 \\ 


%% Our results

%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
%  Multilevel knowledge transfer for crossdomain object detection
% 50.2 whats the venue ?
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% Cross-Domain Adaptive Teacher for Object Detection -*** uses ResNet 101 backbone for detector
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% H2FA R-CNN: Holistic and Hierarchical Feature Alignment for Cross-domain Weakly Supervised Object Detection -*** Does not report foggy citycsapes results in table (only in barplots)
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% Cross Domain Object Detection by Target-Perceived Dual Branch Distillation - *** uses FPN in detector backbone that gives around +5-6 % mAP & performs inference on larger resolution so it is largerly unfair 
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------
% https://arxiv.org/pdf/2212.01322v1.pdf - MIC: Masked Image Consistency for Context-Enhanced Domain Adaptation  - has it been published somewhere ? mAP 47.6 
%% ------------------------------------------------------------------------------------------------------
%% ------------------------------------------------------------------------------------------------------



\\

%bus bcycle car cycle person rider train truck mAP
%(\textit{Ours}) &  & - & - & - & - & - & - & - & - & \textbf{46.9} & - \\



\end{tabular}
\end{adjustbox}
\caption{Adaptation results for Sim10K $\rightarrow$ Cityscapes.}

\label{tab:results:sim10k} 
\end{table}

==> tables/sim10k_to_cityscapes_v02.tex <==
\begin{adjustbox}{scale=0.5}
\begin{tabular}{l | c c c | c} 
\toprule
Method & D.A. & I2I  & Backbone & $AP_{car} \uparrow$  \\
\hline
HTCN~\cite{chen2020harmonizing} \textsc{\textit{{ }     (CVPR '20) }} & {\hspace{0.7cm} \checkmark}& {  \checkmark}&Vgg-16& 42.5\\
UMT~\cite{deng_li_chen_duan_2021}   \textsc{\textit{{ }     (CVPR '21) }} & {\hspace{0.7cm} \checkmark} & {  \checkmark}   &Vgg-16&  43.1\\
FGRR~\cite{DBLP:journals/pami/ChenLZHHDY23} \textsc{\textit{{ }     (PAMI '23) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 44.5\\ 
DSS~\cite{wang2021domain} \textsc{\textit{{ }     (CVPR '21) }}  &  {\hspace{0.7cm} \checkmark}  & &Res-50 & 44.5 \\
SWDA~\cite{saito_ushiku_harada_saenko_2019} \textsc{\textit{{ }     (CVPR '19) }}  & {\hspace{0.7cm} \checkmark}  & &Res-50  & 44.6\\
SCDA~\cite{zhu_pang_yang_shi_lin_2019} \textsc{\textit{{ }     (CVPR '19) }}   & {\hspace{0.7cm} \checkmark}  & &Res-50&   45.1 \\
AFAN~\cite{wang_liao_shao_2021} \textsc{\textit{{ }     (TIP '21) }} & {\hspace{0.7cm} \checkmark}  &   {  \checkmark}& Res-50 & 45.5\\
GPA~\cite{xu2020cross} $(CVPR '20)$  &  {\hspace{0.7cm} \checkmark}   &    & Res-50 & 47.6 \\
SDA~\cite{rezaeianaran2021seeking} \textsc{\textit{{ }     (CVPR '21) }} &{\hspace{0.7cm} \checkmark}&    & Vgg-16& 49.3  \\
MGA~\cite{DBLP:journals/pami/ChenLZHHDY23} \textsc{\textit{{ }     (CVPR '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 49.8\\
KTNet~\cite{9710025} \textsc{\textit{{ }     (ICCV '21) }}&  {\hspace{0.7cm} \checkmark} &&Vgg-16& 50.7 \\
SSAL~\cite{Munir2021SynergizingBS} \textsc{\textit{{ }     (NeurIPS '21) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 51.8\\
SCAN~\cite{DBLP:conf/aaai/LiLYY22} \textsc{\textit{{ }     (AAAI '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 52.6\\
SIGMA~\cite{li2022sigma} \textsc{\textit{{ }     (CVPR '22) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& 53.4\\
DA-DETR~\cite{Zhang2021DADETRDA} \textsc{\textit{{ }     (CVPR '23) }} & {\hspace{0.7cm} \checkmark}&&Vgg-16& \textbf{54.7}\\
\hline
\emph{Source} & && Res-50 & 41.7 \\
Ours - supervised & &{  \checkmark}& Res-50 &  \underline{53.6} \\ 
Ours -  local-global $^{\dag}$   & &{  \checkmark}& Res-50 & 52.1 \\ 
\bottomrule
\end{tabular} 
\end{adjustbox}
\caption{Sim10K $\rightarrow$ Cityscapes.}
\label{tab:results:sim10k} 
